Multimodal Industrial Anomaly Detection by Crossmodal Feature Mapping

The paper explores the industrial multimodal Anomaly Detection (AD) task, which exploits point clouds and RGB images to localize anomalies. We introduce a novel light and fast framework that learns to map features from one modality to the other on nominal samples. At test time, anomalies are detected by pinpointing inconsistencies between observed and mapped features. Extensive experiments show that our approach achieves state-of-the-art detection and segmentation performance in both the standard and few-shot settings on the MVTec 3D-AD dataset while achieving faster inference and occupying less memory than previous multimodal AD methods. Moreover, we propose a layer-pruning technique to improve memory and time efficiency with a marginal sacrifice in performance.

==> sec/2_related_work_old.tex <==
\section{Related Work}
\label{sec:related_work}
 %
\begin{figure*}[ht]
    \centering
        \includegraphics[width=0.88\linewidth]{images/architecture_full.jpg}
    \caption{\textbf{Proposed pipeline.} Given an RGB Image $I_{2D}$ and a Point Cloud $P_{3D}$: a pair of feature extractors,  $\mathcal{F}_{2D},\mathcal{F}_{3D}$,  extract pixel-aligned features maps, $E_{2D},E_{3D}$, by Transformer architectures. Then, a pair of crossmodal feature mappings, $\mathcal{M}_{2D \to 3D}, \mathcal{M}_{3D \to 2D}$, map the extracted features from one modality to the other, processing the features at each pixel independently. Lastly, extracted, $E_{2D},E_{3D}$ and mapped, $\hat{E}_{3D},\hat{E}_{3D}$, features are compared through a discrepancy function $\mathcal{D}$, to create modality-specific anomaly maps, $\Psi_{2D},\Psi_{3D}$, that are then combined by an aggregation function, $\mathcal{A}$, to obtain the final anomaly map $\Psi$.}
    \label{fig:architecture}
\end{figure*}
%

    \noindent
    \textbf{Unsupervised Image Anomaly Detection.}
        % what is unsupervised image AD
        %Unsupervised image AD approaches can be divided into two broad categories, the first operating on the image (pixel) level while the second on feature embeddings.
        Unsupervised AD approaches~\cite{liu2023deep} analyzing RGB Images can be divided into two broad categories.
        The general idea behind the first is to learn how to reconstruct images of nominal samples using auto-encoders~\cite{bergmann2018improving,zavrtanik2021draem,hou2021divide,ristea2022self}, in-painting~\cite{pirnay2022inpainting}, or diffusion models~\cite{wyatt2022anoddpm}. 
        Then, at test time, as the trained model cannot correctly reconstruct anomalous images, a per-pixel anomaly map can be computed by analyzing the discrepancy between the input and reconstructed image.
        %The feature embedding techniques operate on the feature space of deep neural networks.
        The second category of approaches focuses instead on the feature space defined by deep neural networks~\cite{reiss2021panda, yi2020patch, zhang2021anomaly, sohn2021learning, yoa2021self, li2021cutpaste, yang2023memseg, massoli2021mocca, yu2021fastflow, rudolph2021same, rippel2021modeling, gudovskiy2022cflow, chiu2023self, defard2021padim}.
        % teacher-student
        Among these techniques, teacher-student~\cite{bergmann2020uninformed, wang2021student_teacher, cao2022informative, salehi2021multiresolution, deng2022anomaly} is one of the typical strategies employed for AD. 
        During training, the teacher model extracts features from nominal samples and distils the knowledge to the student model. 
        At test time, anomalies are detected by analysing the discrepancy between the features computed by the teacher and the student. 
        % deep reconstruction net
        Differently, Deep Feature Reconstruction (DFR)~\cite{yang2020dfr} trains an auto-encoder on the features extracted from nominal samples. 
        Then, similarly to image reconstruction methods, it identifies anomalies in the test samples by analysing the difference between reconstructed and original features.
        % % one class classification 
        % Other approaches cast AD as a One Class Classification (OCC) problem, in which a classifier is trained to detect nominal samples using unsupervised techniques~\cite{reiss2021panda,yi2020patch,zhang2021anomaly,sohn2021learning} or by generating synthetic anomalies~\cite{yoa2021self,li2021cutpaste,yang2023memseg, massoli2021mocca}.
        % % distribution mapping
        % Distribution mapping techniques try to map complex feature distributions into known ones, such as Gaussians~\cite{yu2021fastflow, rudolph2021same, rippel2021modeling, gudovskiy2022cflow, chiu2023self, defard2021padim}.
        % memory bank
        The increasing availability of effective, general-purpose feature extractors~\cite{caron2021emerging, oquab2023dinov2,he2022masked}, also referred to as \emph{foundation models}, has fostered interest in anomaly detection methods that deploy features extracted by frozen models~\cite{patchcore2022roth,Cohen2020SubImageAD,bergman2020deep}. 
        %based on convolutional architectures~\cite{resnet} or Transformers~\cite{kolesnikov2021vit}, trained on large datasets (e.g., ImageNet~\cite{deng2009imagenet}, SA-1B~\cite{kirillov2023segany}) in a supervised or self-supervised manner (e.g.,~\cite{caron2021emerging, oquab2023dinov2,he2022masked}), 
        At training time, the features computed from nominal samples by a frozen extractor are stored in a memory bank. 
        At inference time, the features extracted from the input image by the frozen model are compared to those stored in the bank to identify anomalies. 
        These approaches achieve remarkable performance, albeit at the cost of slow inference --- since each feature vector extracted from the input image has to be compared to all the nominal ones stored in the bank --- and significant memory occupancy --- since larger memory banks better capture the variability of nominal features. 
        
        %Ours
       %Analogously to~\cite{yang2020dfr}, we deploy a reconstruction objective in feature space. Yet, we focus on multimodal AD and propose a novel crossmodal reconstruction paradigm. 
        
        %We share with   ~\cite{patchcore2022roth,Cohen2020SubImageAD,bergman2020deep} the idea of gathering features from frozen models but, thanks ti to scenario approach also operates in the deep feature space and, similarly to, pursues a reconsitcyon approach. Howecer, how recinstrction happns across modalitire. We share with mmeory-bnks methdos the idea of reliege ob frozen funraui midels but, unklike, we do nor rely on memiry banks. 

       %Our approach also operates in the deep feature space. However, differently from the solutions described above we focus on the multimodal AD scenario.

    \noindent
    \textbf{Multimodal RGB-3D Anomaly Detection.}
        Multimodal approaches exploit both RGB images and 3D data to enhance the robustness and effectiveness of anomaly detection.  
        %
        %Following the influential work on benchmarking image-based AD~\cite{bergmann2019mvtec}, a recent paper~\cite{bergmann2022mvtec} has introduced the MVTec 3D-AD dataset, alongside an experimental validation including several baselines. These baselines have been trained on 3D data represented by voxel grids or depth maps and RGB information incorporated as additional input channels.
        Following the influential work on benchmarking image-based AD~\cite{bergmann2019mvtec}, a recent paper~\cite{bergmann2022mvtec} has introduced the MVTec 3D-AD dataset, alongside an experimental validation including several baselines, such as distribution mapping techniques based on GANs and variational models (\ie, VAEs), as well as auto-encoders. 
        These baseline models are trained on 3D data represented by voxel grids or depth maps and incorporate RGB information as additional input channels.
        %
        The method proposed in~\cite{RudWeh2023} consists of an asymmetric student-teacher approach (AST) aimed at processing RGB-D data, in which the two networks have different architectures to prevent over-generalization on anomalous samples. % typical of teacher-student techniques.
        %
        Inspired by PatchCore~\cite{patchcore2022roth}, BTF~\cite{horwitz2023back} investigates the use of memory banks for 3D anomaly detection.
        The authors propose to add 3D features to the 2D features provided by a frozen convolutional model (Wide ResNet-50) to enhance anomaly detection performance.
        They test several 3D features and achieve the best results using hand-crafted descriptors extracted from Point Clouds~\cite{fpfh}.
        %
        M3DM~\cite{wang2023multimodal} improved over BTF by employing rich and distinctive 2D and 3D features extracted by frozen Transformer-based foundation models trained by self-supervision on large datasets. 
        In particular, they use DINO~\cite{caron2021emerging} and Point-MAE~\cite{pang2022masked} to extract 2D and 3D features, respectively. 
        The authors also propose a learned function to fuse 2D and 3D features into multimodal features stored in memory banks alongside those computed from the individual modalities. 
        Thanks to the joint deployment of powerful 2D, 3D and multimodal features, they achieve excellent performance, setting the highest bar on MVTec 3D-AD. 
        However, reliance on large feature banks renders M3DM overly expensive in terms of memory and time (\cref{fig:teaser}). 
        %  necessitates of comes at the cost of  relies on a very large memory   % and, a Transformer encoder for Point Clouds trained by  a masked reconstruction objective inspired by~\cite{he2022masked}.  
        %to extract   and larger memory banks. 
        %Even though this method achieves outstanding performance, it demands substantial memory capacity and exhibits slow inference speeds.
        %d RIVEDERRE DA QUI
        Similarly to M3DM~\cite{wang2023multimodal}, our method deploys compelling 2D and 3D features computed by frozen Transformer-based models. Yet, we do not employ any memory bank and, instead, propose a novel crossmodal feature mapping paradigm that can be realized by two lightweight neural networks. 
        Using the same feature extractors as M3DM~\cite{wang2023multimodal}, we achieve better performance on MVTec 3D-AD while requiring way less memory and running remarkably faster (\cref{fig:teaser}).
        % EasyNet~\cite{chen2023easynet}

==> sec/3_method_old.tex <==
\section{Method}
\label{sec:method}
    Our proposed AD approach relies on learning  to predict crossmodal mappings between features extracted from nominal samples in order to pinpoint anomalies based on the discrepancy between predicted and observed features (\cref{fig:architecture}). As pointed out in \cref{sec:introduction}, this novel paradigm offers high sensitivity toward all kinds of anomalies. Let us conceptualize this property  with the aid of the toy examples presented in \cref{fig:sketch}.
    At training time (top left) we observe red 2D patches on flat 3D patches and blue 2D patches on curved 3D patches:   $\mathcal{M}_{2D \to 3D}$ and $\mathcal{M}_{3D \to 2D}$ learn to predict the relationships between the features extracted from these patches. At inference time, if an anomalous, e.g. yellow, 2D patch appears on a curved surface  (top right, 2D-Only Anomaly), $\mathcal{M}_{3D \to 2D}$ predicts the 2D feature corresponding to a blue patch, whilst the observed 2D feature concerns a yellow patch. Moreover, $\mathcal{M}_{2D \to 3D}$ receives an input feature unseen at training time, which would unlikely yield as output the 3D feature of the actual curved patch. Thus, our method senses discrepancy between prediction and observation for both the 2D and the 3D features. %For both predictions to agree with the observations, $\mathcal{M}_{3D \to 2D}$ should predict a feature never seen at training time, i.e that of a yellow patch, and $\mathcal{M}_{2D \to 3D}$ return exactly the feature of the curved surface, both circumstances  being unlikely. 
    Similar considerations do apply to the case of a nominal 2D patch on an anomalous 3D patch (bottom right, 3D-Only Anomaly): both predictions disagree with the observations. This is the case also when both modalities exhibit anomalies (not shown in \cref{fig:sketch}): both inputs are unseen at training time and so both crossmodal predictions are unlikely to match the observations. Finally, we highlight the case mandating multimodal AD: the individual modalities comply with the nominal distributions but their co-occurrence is anomalous. 
    In our conceptualization, this may be exemplified by a red patch on a curved surface  (bottom left, Multimodal-Only Anomaly): again, as $\mathcal{M}_{2D \to 3D}$ outputs the 3D feature of the flat patch and $\mathcal{M}_{3D \to 2D}$ the 2D feature of the blue one, both predictions disagree with the observations. 

    It is worth pointing out that, due to the variability of the nominal samples, the mappings between 2D and 3D features  may not be \emph{unique}. For instance, in  \cref{fig:sketch}, there might be both flat and curved surfaces coloured in red, this \emph{one-to-many} mapping making it impossible for $\mathcal{M}_{2D \to 3D}$ to learn the correct 3D feature to be associated to the 2D feature of a red patch. As a consequence, when presented with a red patch  $\mathcal{M}_{2D \to 3D}$ may predict either the wrong 3D feature or an unlikely one, thereby causing a discrepancy between the predicted and observed 3D features. Yet, $\mathcal{M}_{3D \to 2D}$ can  predict the 2D feature of the red patch, due to the   $3D \to 2D$ mapping being \emph{many-to-one}. Thus, we may avoid a false detection by pinpointing anomalies only  when both predictions  disagree with the observations. Of course, due to even higher variability across nominal samples, we may also face \emph{one-to-many}  $3D \to 2D$ mappings, e.g. considering again  \cref{fig:sketch}, both blue and red image patches on curved 3D  patches. In such a case, when presented with a red patch on a curved surface $\mathcal{M}_{2D \to 3D}$ may wrongly predict the feature of a flat 3D patch and $\mathcal{M}_{3D \to 2D}$ that of a blue 2D patch, ending up in  a false anomaly detection due to both predictions --- wrongly --- disagreeing with observations.  
            
    Nonetheless, in our framework, we can address the issue of potential  \emph{one-to-many} feature mappings across modalities  by leveraging on the highly contextualized 2D and 3D features provided by Transformer architectures~\cite{caron2021emerging, pang2022masked}. Indeed, a contextualized 2D feature, e.g. describing a red patch surrounded by blue and purple patches, tends to correspond to a specific contextualized 3D feature, e.g. representing a flat patch just to the right to a rippling surface area. In other words, the highly contextualized  2D and 3D features extracted by Transformers are less prone to realize \emph{one-to-many} crossmodal mappings.  
   
    
    %It is worth pointing out that the mappings between 2D and 3D features across nominal samples may not be \emph{unique}: e.g., in the previous example, there might be both flat and curved surfaces coloured in red, which would make it impossible for $\mathcal{M}_{2D \to 3D}$ to learn the correct 3D feature to be associated to the 2D feature of a red patch. In our framework, we address this issue effectively by leveraging on the highly contextualized 2D and 3D features provided by Transformer architectures~\cite{caron2021emerging, pang2022masked}. Indeed, a contextualized 2D feature, e.g. describing a red patch surrounded by blue and purple patches, tends to correspond to a specific contextualized 3D feature, e.g. representing a flat patch just to the right to a rippling surface area. In other words, the highly contextualized  2D and 3D features extracted by Transformers are less prone to realize \emph{one-to-many} crossmodal mappings.  
    

    
   % perduct the feature of curved 3D òpatch: thus an anmaly in 2D woudlyield discrepanceis between bisrced na orducetd fetayre fir bith th maoing netword, 
    
    %onsider an RGB-only anomaly. In this case, by mapping 3D features to the RGB space, we obtain a nominal RGB feature different from the one extracted from the anomalous data. At the same time, the opposite mapping network from RGB to 3D fails as input features are out of the nominal distribution. Thus, we can easily detect this kind of anomaly.
    %Another scenario is a strictly multimodal anomaly. Let us imagine that in nominal samples, features of red RGB patches are associated with flat surfaces, but the anomaly sample has a red curved surface.
    %Yet, curved surfaces also appear in nominal samples. Thus, we would not be able to detect this anomaly from 3D-only information. Our method can correctly identify such anomalies because the red RGB feature is mapped to a flat surface feature, not a curved one.
    
    %such as discrepancues i.e. unseen pairings   We propose a crossmodal approach to effectively combine 2D and 3D information, enhancing both detection and segmentation performances with respect to the state-of-the-art.  and
    %The method is also swift and requires no external memory banks for inference or training.
    
    The proposed method is thoroughly introduced in this section.
    As depicted in \cref{fig:architecture}, the method consists of \emph{(i)} a pair of pre-trained \emph{Feature Extractors} (FEs); \emph{(ii)} a pair of \emph{Feature Mappings} (FMs); and \emph{(iii)} an \emph{Aggregation Module} (AM).
    The Aggregation Module is employed only at inference time.
    
    \begin{figure}[t]
        \centering
            \includegraphics[width=\linewidth]{images/sketch_explanation.jpg}
        \caption{\textbf{Type of anomalies.}}
        \label{fig:sketch}
    \end{figure}

    \subsection{Overview} 
        The method takes as inputs an RGB Image $I_{2D}$ and the corresponding pixel-aligned Point Cloud $P_{3D}$ to perform anomaly detection and segmentation, hence producing an anomaly map $\Psi : \mathbb{R}^2 \to \mathbb{R}$ and a global anomaly score $\psi \in \mathbb{R}$.
    
        At training time, a couple of Feature Extractors $\mathcal{F}_{2D}, \mathcal{F}_{3D}$ extracts feature maps $E_{2D}, E_{3D}$ from the respective modalities of train samples --- which can be only nominal ---
        %(e.g. DINO extracts a RGB features map, while Point-MAE extracts a Point Cloud features map) 
        while a couple Feature Mappings $\mathcal{M}_{2D \to 3D}, \mathcal{M}_{3D \to 2D}$ is trained to predict the corresponding feature $\hat{E}_{3D}, \hat{E}_{2D}$ from the other modality in a reconstruction fashion.

        At inference time, test samples --- which can be either nominal or anomalous --- are forwarded to the Feature Extractors and the Feature Mappings, obtaining two pairs of extracted and reconstructed embeddings $(E_{2D}, \hat{E}_{2D}), (E_{3D}, \hat{E}_{3D})$.
        Each pair is then compared separately with a distance function $\mathcal{D}$, obtaining two anomaly maps $\Psi_{2D}, \Psi_{3D}$.
        In the end, the two anomaly maps are aggregated with an aggregation function $\mathcal{A}$, to obtain a comprehensive anomaly map $\Psi$, from which also a global anomaly score $\psi$ is extracted.

        The idea behind this approach is that, at training time, the Feature Mappings learn to reconstruct the features of nominal samples, hence, at test time, when a nominal sample is presented the FMs will be able to reconstruct it, while when an anomalous sample is provided the FMs will falter to reconstruct it correctly, suggesting an anomaly in the sample.
        It is worth noting that, by letting the FMs reconstruct the corresponding feature from different modalities, the risk of learning the identity function, which hinders the anomaly detection and segmentation performance, is mitigated.

    \subsection{Crossmodal Mapping}
        \subsubsection{Feature Extractors}
            A Feature Extractor is a function $\mathcal{F}: \mathbb{R}^{H \times W \times 3} \to \mathbb{R}^{S \times D}$ that maps RGB Images or Point Clouds into sequences of feature embeddings with dimensionality $D$ and sequence length $S$.
            %
            \begin{equation}
                E_{2D} = \mathcal{F}_{2D}(I_{2D}) \quad E_{3D} = \mathcal{F}_{3D}(P_{3D})
            \end{equation}
            %
            Such function can be either determined with handcrafted algorithms, as in PCA, or learned from the data, as in convolutional networks and transformers.

        \subsubsection{Feature Alignment}
            A Point Transformer \cite{zhao2021point} and an Image Transformer \cite{kolesnikov2021vit} are employed as FEs to extract features from Point Clouds and RGB Images, respectively.
            Since each FE can have different sequence lengths, as well as hidden space dimensions, a procedure to align the Point Transformer feature to a 2D plane, introduced by \cite{wang2023multimodal}, is used.
            
            Each Point Cloud $P_{3D}$ is sampled with a Farthest Point Sampling (FPS) \cite{pointent2}, which partitions the $N$ points into $G$ groups with $n$ points each.
            The points in each group are then encoded into a feature vector, and the $G$ vectors are input into the Point Transformer. 
            The output $E_{3D}$ of the Point Transformer $\mathcal{F}_{3D}$ are, thus, $G$ point features, which can be seen as the features of the center point of each group.
            After the FPS, the group center points are not evenly distributed in space, leading to an unbalanced density of point features. 
            To overcome this issue, the features are interpolated back to the original Point Cloud by inverse distance weighting.
            % Vedi equazione M3DM.
            After the interpolation, the re-weighted features are projected onto the 2D plane using the point coordinates and camera parameters. 
            Since the Point Clouds could be sparse, if a 2D plane position does not match any point, the corresponding position is set as 0.
            In the end, an average pooling operation is employed to get the patch feature on the 2D plane feature map.

             
        \subsubsection{Feature Mappings}
            A Feature Mapping is a function $\mathcal{M}: \mathbb{R}^{S \times D_{A}} \to \mathbb{R}^{S \times D_{B}}$ which translates feature embeddings from a feature space with dimensionality $D_{A}$ to another one with dimensionality $D_{B}$.
            In the context of this work, we aim to translate previously extracted 2D features to 3D features and vice versa.
            %
            \begin{equation}
                \hat{E}_{3D} = \mathcal{M}_{2D \to 3D}(E_{2D}) \quad \hat{E}_{2D} = \mathcal{M}_{3D \to 2D}(E_{3D})
            \end{equation}
            %
            The Feature Mappings are jointly optimized by minimizing the cosine distance between the original feature vector and the reconstructed one.
            %
            \begin{equation}
                \begin{split}
                    \mathcal{L}(E, \hat{E}) & = \mathcal{L}_{2D \to 3D}(E_{2D}, \hat{E}_{2D}) + \mathcal{L}_{3D \to 2D}(E_{3D}, \hat{E}_{3D}) \\
                                            & = \bigl(1 - S_C (E_{2D}, \hat{E}_{2D})\bigr) + \bigl(1 - S_C (E_{3D}, \hat{E}_{3D})\bigr) \\
                                            & = \Biggl(1 - \frac{E_{2D} \cdot \hat{E}_{2D}}{\|E_{2D}\|  \|\hat{E}_{2D}\|}\Biggr) + \Biggl(1 - \frac{E_{3D} \cdot \hat{E}_{3D}}{\|E_{3D}\| \|\hat{E}_{3D}\|}\Biggr)
                \end{split}
            \end{equation}
            %
            
        \subsubsection{Aggregation Module}
            At inference time, test samples --- which can be either nominal or anomalous --- are forwarded to the Feature Extractors and the Feature Mappings, obtaining two couples of extracted and reconstructed embeddings $(E_{2D}, \hat{E}_{2D}), (E_{3D}, \hat{E}_{3D})$.
            
            Each couple is compared independently with a distance function $\mathcal{D}$, obtaining two anomaly maps $\Psi_{2D}, \Psi_{3D}$.
            %
            \begin{equation}
                \Psi_{2D} = \mathcal{D}(E_{2D}, \hat{E}_{2D}) \quad \Psi_{2D} = \mathcal{D}(E_{3D}, \hat{E}_{3D})
            \end{equation}
            %
            In the context of this work, the Euclidean distance on normalized embeddings is employed.
            %
            \begin{equation}
                \mathcal{D}(E', E'') = \Biggl\|\frac{E'}{\|E'\|_{2}} - \frac{E''}{\|E''\|_{2}}\Biggr\|_{2}
            \end{equation}
            %
            Then, with an aggregation function $\mathcal{A}$ a comprehensive anomaly map $\Psi$ is obtained.
            %
            \begin{equation}
                \Psi = \mathcal{A}(\Psi_{2D}, \Psi_{3D})
            \end{equation}
            %
            Additionally, the resulting anomaly map is smoothed with a Gaussian of kernel width $\sigma = 4$, as also performed in previous works~\cite{wang2023multimodal, patchcore2022roth, Cohen2020SubImageAD}.
    
            In the end, the global anomaly score $\psi$ is obtained as the maximum value of the anomaly map $\Psi$.
            %
            \begin{equation}
                \psi = \max(\Psi)
            \end{equation}
            %

        \subsection{Layers Pruning}

            \begin{figure}[ht]
                \centering
                    \includegraphics[width=0.75\linewidth]{images/trasformer_pruning_full.jpg}
                \caption{\textbf{Layers Pruning.} }
                \label{fig:pruning}
            \end{figure}

==> sec/5_experiments_old.tex <==
\section{Experiments}
\label{sec:experiments}

    \subsection{Quantitative Results}
        We compare our method with several multimodal methods on the MVTec 3D-AD dataset: \emph{(i)}~\cref{tab:iauroc_comparisons_mvtec} reports the anomaly detection results with I-AUROC; \emph{(ii)}~\cref{tab:aupro_comparisons_mvtec} reports the anomaly segmentation results with AUPRO; \emph{(iii)}~\cref{tab:pauroc_comparisons_mvtec} reports the anomaly segmentation results with P-AUROC. 
        These comparisons are also reported for the Eyecandies dataset in the Supplementary Material.
        We identify M3DM as our main competitor.
        Our method achieves the best results in both detection and segmentation, by outperforming of 0.7\% the previous best AUPRO score by M3DM, of 0.9\% the previous best I-AUROC score by M3DM and of 0.1\% the previous P-AUROC score by M3DM and BTF.
        However, we would like to highlight that P-AUROC is a saturated metric.

        \input{tables/iauroc_comparisons_mvtec}

        \input{tables/pauroc_comparisons_mvtec}

        \input{tables/aupro_comparisons_mvtec}

        \input{tables/ftn_fpr-rate_ablation}

    \subsection{Qualitative Results}
        In~\cref{fig:qualitatives_mvtec} the qualitative results on some classes of the MVTec 3D-AD dataset are shown. 
        % Commento sui risultati e comparison con M3DM.
        More extensive results are presented in the Supplementary Material.
        \input{figures/qualitatives_mvtec}

    \subsection{Memory Occupancy and Inference Speed}
        Other AD methods, such as BTF~\cite{horwitz2023back} and M3DM~\cite{wang2023multimodal}, construct large memory banks of features, at the cost of high memory consumption and long inference times, as shown in~\cref{tab:time-space_performance}.
        AST~\cite{RudWeh2023} mitigates the memory occupancy problem by not employing memory banks but is still rather slow due to its Normalizing Flow architecture.
        Our approach overcomes both issues by employing MLPs as Feature Mappings, achieving a real-time inference speed with the lighter version.
        More thorough results are described in~\cref{subsubsec:ftn_layers_ablation}.
        
        \input{tables/time-space_performance}

    \subsection{Ablation Study}

        \textbf{Analysis of False Positive Rate in AUPRO.}
            As anticipated in~\cref{subsec:metric}, we argue that a $30\%$ threshold for false positive rate is too permissive for an actual industrial application, therefore we re-evaluate previous benchmarks with a more restrictive rate.
            As depicted in~\cref{tab:aupro_fpr-rate_mvtec} the proposed method achieves the best performance also in this more difficult benchmark.
            
        \textbf{Analysis of Aggregation Function.}
            \label{subsubsec:ftn_aggregation_ablation}
            At inference time, the method produces a distinct anomaly map for each modality.
            We investigate several methods to combine such maps to obtain the final aggregated anomaly map, such as: \emph{(i)} computing the product of the two anomaly maps; \emph{(ii)} taking the pixel-wise maximum of each modality; \emph{(iii)} summing the two anomaly maps.
            Following the results presented in~\cref{tab:ftn_modality-aggregation_ablation} it is observable how taking the product of the two modalities achieves the best performance in both detection and segmentation tasks.
            We argue that this behaviour is consistent with the fact that, by taking the product of the two anomaly maps, a logical and is enforced between the two maps, hence only the defects confirmed by both modalities are considered anomalous.
            %Performed on the best model.
            \input{tables/ftn_modality-aggregation_ablation}
            
        \textbf{Analysis of Modality Contribution.}
            \label{subsubsec:ftn_modality_ablation}
            At inference time, the method produces a distinct anomaly map for each modality.
            We explore the importance of combining both these modalities to achieve the best performance. 
            In~\cref{tab:ftn_modality-aggregation_ablation} detection and segmentation metrics are calculated by considering the following scenarios: \emph{(i)} evaluation of the 2D-only anomaly map; \emph{(ii)} evaluation of the 3D-only anomaly map; \emph{(iii)} evaluation of the aggregated anomaly map, aggregated accordingly to what has been shown in~\cref{subsubsec:ftn_aggregation_ablation}.
            From this experiment, it is evident how the best choice is to combine the two anomaly maps, since the latter scenario consistently achieves a better performance, across all the dataset classes.
            
        \textbf{Analysis of Crossmodality Contribution.}
            The core idea of our method is that by reconstructing the features from a feature space to another we are able to avert the risk of learning the identity function, typical of reconstruction-based methods, which hinders detection and segmentation performance.
            In~\cref{tab:ftn_crossmodality_ablation} the comparison between reconstructing the same modality and crossing them is shown, as well as evaluating a single modality when the same modality is reconstructed.
            The results show once again, as already observed in~\cref{subsubsec:ftn_modality_ablation}, that combining the two anomaly maps helps in both detection and segmentation task, and also that crossing the modalities enhance the performance as well.
            
            \input{tables/ftn_crossmodality_ablation}

        \textbf{Analysis of Feature Extractors Layers.}
            \label{subsubsec:ftn_layers_ablation}
            We explore the possibility of training the Feature Mappings on different levels of each transformer output, to achieve faster and lighter models.
            We train the FMs after the 1st, 4th, 8th and last layer of both transformers and we denote each model respectively as \emph{Tiny}, \emph{Small}, \emph{Medium} and \emph{Base}.
            ~\cref{tab:time-space_performance} depicts that with the \emph{Small} and \emph{Medium} models, we achieve a significant speed-up and reduced memory occupancy while still retaining state-of-the-art performances. 
            With the \emph{Tiny} model, we still achieve state-of-the-art performance in anomaly segmentation with a slight drop in performance in anomaly detection, while also being able to run the algorithm in real-time.
                    
        \textbf{Analysis of Feature Extractors.}
            \label{subsubsec:fe_ablation}
            We investigate the use of several popular RGB transformer-based backbones, among them: SAM~\cite{kirillov2023segany}, CLIP~\cite{radford2021learning}, DINO-v2~\cite{oquab2023dinov2}.
            ~\cref{tab:ftn_backbone_ablation} shows that DINO and DINO-v2 exhibit the best performance.
            We observe that the ones pre-trained with a self-supervised contrast learning approach beget better performance in the task.
            
            \input{tables/ftn_backbone_ablation}
            
        \textbf{Analysis of Few-shot Learning.}
            We investigate the few-shot capabilities of the method. We randomly select 50, 10 and 5 images from each category as training data and test the few-shot model on the full dataset, as shown in~\cref{tab:ftn_few-shot_mvtec}.
            We observe that the method, in all the few-shot settings, has a better segmentation performance than the other methods, while it achieves comparable detection performance to M3DM~\cite{wang2023multimodal}.
            
            \input{tables/ftn_few-shot_ablation}

==> tab_no-align.tex <==
\begin{comment}
\begin{table}[]
    \centering
    \resizebox{0.5\textwidth}{!}{%
    \begin{tabular}{c||cccccccccc||c}

        \textbf{Method} &
        \textit{Bagel} &
        \textit{Cable Gland} &
        \textit{Carrot} &
        \textit{Cookie} &
        \textit{Dowel} &
        \textit{Foam} &
        \textit{Peach} &
        \textit{Potato} &
        \textit{Rope} &
        \textit{Tire} &
        \textbf{Mean} \\ 

        \hline
        
        AUPRO@30\% & 0.684 & 0.771 & 0.924 & 0.511 & 0.835 & 0.539 & 0.857 & 0.899 & 0.795 & 0.676 & 0.749 \\
        AUPRO@10\% & 0.369 & 0.428 & 0.772 & 0.200 & 0.510 & 0.326 & 0.623 & 0.697 & 0.482 & 0.345 & 0.475 \\
        AUPRO@5\%  & 0.224 & 0.250 & 0.571 & 0.100 & 0.257 & 0.217 & 0.463 & 0.485 & 0.289 & 0.195 & 0.305 \\
        AUPRO@1\%  & 0.055 & 0.061 & 0.181 & 0.017 & 0.051 & 0.076 & 0.177 & 0.155 & 0.081 & 0.045 & 0.090 \\

        \hline
        
        P-AUROC    & 0.904 & 0.931 & 0.977 & 0.843 & 0.951 & 0.837 & 0.960 & 0.972 & 0.943 & 0.900 & 0.922 \\
        I-AUROC    & 0.601 & 0.489 & 0.604 & 0.476 & 0.538 & 0.632 & 0.601 & 0.528 & 0.558 & 0.537 & 0.556 \\

        \hline
        
    \end{tabular}}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
\end{comment}

==> tables/aupro_comparisons_eyecandies.tex <==
\begin{table*}
    \centering
    \resizebox{0.75\textwidth}{!}{%
        \begin{tabular}{c||cccccccccc||c}

            \textbf{Method} &
            \textit{Can. C.} &
            \textit{Cho. C.} &
            \textit{Cho. P.} &
            \textit{Conf.} &
            \textit{Gum. B.} &
            \textit{Haz. T.} &
            \textit{Lic. S.} &
            \textit{Lollip.} &
            \textit{Marsh.} &
            \textit{Pep. C.} &
            \textbf{Mean} \\

            \hline

            M3DM~\cite{wang2023multimodal} & 0.906 & 0.923 & 0.803 & 0.983 & 0.855 & 0.688 & 0.880 & 0.906 & 0.966 & 0.955 & 0.882 \\
            Ours                           & 0.942 & 0.902 & 0.831 & 0.965 & 0.875 & 0.762 & 0.791 & 0.913 & 0.939 & 0.949 & 0.887 \\
            
            \hline
            
        \end{tabular}}
    \caption{\textbf{AUPRO@30\% on Eyecandies dataset with several AD methods.} Best results in \textbf{bold}, runner-ups \underline{underlined}.}
    \label{tab:aupro_comparisons_eyecandies}
\end{table*}

==> tables/aupro_comparisons_mvtec.tex <==
\begin{table*}[h]
    \centering
    \resizebox{0.75\textwidth}{!}{%
        \begin{tabular}{c||cccccccccc||c}

            \textbf{Method} &
            \textit{Bagel} &
            \textit{Cable Gland} &
            \textit{Carrot} &
            \textit{Cookie} &
            \textit{Dowel} &
            \textit{Foam} &
            \textit{Peach} &
            \textit{Potato} &
            \textit{Rope} &
            \textit{Tire} &
            \textbf{Mean} \\ 

            \hline

            DepthGAN~\cite{bergmann2022mvtec} & 0.421 & 0.422 & 0.778 & 0.696 & 0.494 & 0.252 & 0.285 & 0.362 & 0.402 & 0.631 & 0.474 \\
            DepthAE~\cite{bergmann2022mvtec}  & 0.432 & 0.158 & 0.808 & 0.491 & 0.841 & 0.406 & 0.262 & 0.216 & 0.716 & 0.478 & 0.481 \\
            DepthVM~\cite{bergmann2022mvtec}  & 0.388 & 0.321 & 0.194 & 0.570 & 0.408 & 0.282 & 0.244 & 0.349 & 0.268 & 0.331 & 0.335 \\
            VoxelGAN~\cite{bergmann2022mvtec} & 0.664 & 0.620 & 0.766 & 0.740 & 0.783 & 0.332 & 0.582 & 0.790 & 0.633 & 0.483 & 0.639 \\
            VoxelAE~\cite{bergmann2022mvtec}  & 0.467 & 0.750 & 0.808 & 0.550 & 0.765 & 0.473 & 0.721 & 0.918 & 0.019 & 0.170 & 0.564 \\
            VoxelVM~\cite{bergmann2022mvtec}  & 0.510 & 0.331 & 0.413 & 0.715 & 0.680 & 0.279 & 0.300 & 0.507 & 0.611 & 0.366 & 0.471 \\
            BTF~\cite{horwitz2023back}        & \underline{0.976} & 0.969 & 0.979 & \textbf{0.973} & 0.933 & 0.888 & 0.975 & \underline{0.981} & 0.950 & 0.971 & 0.959 \\
            AST~\cite{RudWeh2023}             & 0.970 & 0.947 & \underline{0.981} & 0.939 & 0.913 & 0.906 & \underline{0.979} & \textbf{0.982} & 0.889 & 0.940 & 0.944 \\
            M3DM~\cite{wang2023multimodal}    & 0.970 & \underline{0.971} & 0.979 & \underline{0.950} & \underline{0.941} & \underline{0.932} & 0.977 & 0.971 & \underline{0.971} & \underline{0.975} & \underline{0.964} \\
            % EasyNet~\cite{chen2023easynet}    & 0.839 & 0.864 & 0.951 & 0.618 & 0.828 & 0.836 & 0.942 & 0.889 & 0.911 & 0.528 & 0.821 \\
            Ours                              & \textbf{0.979} & \textbf{0.972} & \textbf{0.982} & 0.945 & \textbf{0.950} & \textbf{0.968} & \textbf{0.980} & \textbf{0.982} & \textbf{0.975} & \textbf{0.981} & \textbf{0.971} \\
            
            \hline
            
        \end{tabular}}
    \caption{\textbf{AUPRO@30\% MVTec 3D-AD of multi-modal AD methods..} Best results in \textbf{bold}, runner-ups \underline{underlined}.}
    \label{tab:aupro_comparisons_mvtec}
\end{table*}

==> tables/ftn_aggregation_ablation.tex <==
\begin{table*}
    \centering
    \resizebox{0.75\textwidth}{!}{%
        \begin{tabular}{c||cccccccccc||c}

            \textbf{Metric} &
            \textit{Bagel} &
            \textit{Cable Gland} &
            \textit{Carrot} &
            \textit{Cookie} &
            \textit{Dowel} &
            \textit{Foam} &
            \textit{Peach} &
            \textit{Potato} &
            \textit{Rope} &
            \textit{Tire} &
            \textbf{Mean} \\ 

            \hline

            & \multicolumn{10}{c}{$\Psi_{2D} \cdot \Psi_{3D}$} & \\

            \hline

            I-AUROC   & 0.994 & 0.888 & 0.984 & 0.993 & 0.980 & 0.888 & 0.941 & 0.943 & 0.980 & 0.953 &  0.954 \\            
            P-AUROC   & 0.997 & 0.992 & 0.999 & 0.972 & 0.987 & 0.993 & 0.998 & 0.999 & 0.998 & 0.998 &  0.993 \\

            \hline
            
            AUPRO@30\% & 0.979 & 0.972 & 0.982 & 0.945 & 0.950 & 0.968 & 0.980 & 0.982 & 0.975 & 0.981 &  0.971 \\            
            AUPRO@10\% & 0.937 & 0.917 & 0.947 & 0.897 & 0.855 & 0.906 & 0.942 & 0.947 & 0.926 & 0.944 &  0.922 \\
            AUPRO@5\%  & 0.877 & 0.843 & 0.894 & 0.840 & 0.765 & 0.828 & 0.884 & 0.894 & 0.865 & 0.889 &  0.858 \\
            AUPRO@1\%  & 0.459 & 0.431 & 0.485 & 0.469 & 0.394 & 0.413 & 0.468 & 0.487 & 0.464 & 0.476 &  0.455 \\

            \hline

            & \multicolumn{10}{c}{$\max(\Psi_{2D}, \Psi_{3D}$)} & \\
            
            \hline
            
            I-AUROC   & 0.937 & 0.865 & 0.984 & 0.951 & 0.983 & 0.789 & 0.915 & 0.736 & 0.968 & 0.825 & 0.895 \\
            P-AUROC   & 0.988 & 0.993 & 0.997 & 0.940 & 0.973 & 0.977 & 0.997 & 0.997 & 0.996 & 0.994 & 0.985 \\

            \hline
            
            AUPRO@30\% & 0.960 & 0.966 & 0.979 & 0.884 & 0.911 & 0.916 & 0.981 & 0.974 & 0.958 & 0.971 & 0.950 \\
            AUPRO@10\% & 0.896 & 0.906 & 0.937 & 0.813 & 0.741 & 0.783 & 0.942 & 0.922 & 0.878 & 0.913 & 0.873 \\
            AUPRO@5\%  & 0.819 & 0.834 & 0.874 & 0.738 & 0.624 & 0.675 & 0.884 & 0.844 & 0.789 & 0.841 & 0.792 \\
            AUPRO@1\%  & 0.410 & 0.428 & 0.456 & 0.371 & 0.311 & 0.326 & 0.468 & 0.410 & 0.401 & 0.429 & 0.401 \\
            

            \hline

            & \multicolumn{10}{c}{$\Psi_{2D} + \Psi_{3D}$} & \\

            \hline
            
            I-AUROC   & 0.980 & 0.893 & 0.991 & 0.996 & 0.980 & 0.844 & 0.970 & 0.876 & 0.966 & 0.894 & 0.939 \\
            P-AUROC   & 0.992 & 0.993 & 0.998 & 0.948 & 0.974 & 0.990 & 0.998 & 0.998 & 0.996 & 0.996 & 0.988 \\
            
            \hline
            
            AUPRO@30\% & 0.969 & 0.968 & 0.980 & 0.904 & 0.914 & 0.958 & 0.982 & 0.977 & 0.961 & 0.977 & 0.959 \\
            AUPRO@10\% & 0.917 & 0.912 & 0.941 & 0.853 & 0.749 & 0.877 & 0.945 & 0.932 & 0.886 & 0.931 & 0.894 \\
            AUPRO@5\%  & 0.852 & 0.844 & 0.882 & 0.799 & 0.638 & 0.784 & 0.890 & 0.864 & 0.806 & 0.869 & 0.823 \\
            AUPRO@1\%  & 0.448 & 0.439 & 0.468 & 0.462 & 0.323 & 0.384 & 0.478 & 0.439 & 0.424 & 0.456 & 0.432 \\

            \hline
            
        \end{tabular}}
    \caption{\textbf{Analysis of Aggregation Function.} Results on MVTec 3D-AD. Best results highlighted in \textbf{bold}.}
    \label{tab:ftn_aggregation_ablation}
\end{table*}

==> tables/ftn_backbone_ablation_old.tex <==
\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{c||cccccccccc||c}

            \textbf{Metric} &
            \textit{Bagel} &
            \textit{Cable Gland} &
            \textit{Carrot} &
            \textit{Cookie} &
            \textit{Dowel} &
            \textit{Foam} &
            \textit{Peach} &
            \textit{Potato} &
            \textit{Rope} &
            \textit{Tire} &
            \textbf{Mean} \\ 

            \hline

            & \multicolumn{10}{c}{\textbf{(a) MLP Projection [DINO \& Point-MAE] @50ep}} & \\

            \hline
            
            I-AUROC & 0.990 & 0.894 & 0.986 & 0.989 & 0.980 & 0.916 & 0.951 & 0.916 & 0.986 & 0.886 & 0.949 \\
            P-AUROC & 0.997 & 0.989 & 0.999 & 0.971 & 0.985 & 0.992 & 0.998 & 0.999 & 0.998 & 0.996 & 0.992 \\
            AUPRO@30\% & 0.979 & 0.963 & 0.982 & 0.940 & 0.944 & 0.961 & 0.980 & 0.983 & 0.972 & 0.980 & 0.968 \\
            AUPRO@1\%  & 0.469 & 0.402 & 0.486 & 0.450 & 0.380 & 0.397 & 0.463 & 0.490 & 0.453 & 0.463 & 0.445 \\
            
            \hline

            & \multicolumn{10}{c}{\textbf{(b) MLP Projection [SAM \& Point-MAE] @50ep}} & \\
            
            \hline
            I-AUROC & 0.855 & 0.681 & 0.921 & 0.981 & 0.796 & 0.669 & 0.875 & 0.766 & 0.838 & 0.536 & 0.792 \\
            P-AUROC & 0.991 & 0.944 & 0.997 & 0.965 & 0.973 & 0.906 & 0.994 & 0.995 & 0.993 & 0.971 & 0.973 \\
            AUPRO@30\% & 0.959 & 0.802 & 0.981 & 0.929 & 0.902 & 0.691 & 0.971 & 0.973 & 0.951 & 0.905 & 0.906 \\
            AUPRO@1\%  & 0.348 & 0.162 & 0.473 & 0.402 & 0.258 & 0.156 & 0.386 & 0.424 & 0.332 & 0.173 & 0.311 \\
            
            \hline

            & \multicolumn{10}{c}{\textbf{(c) MLP Projection [DINO-v2 \& Point-MAE] @50ep}} & \\

            \hline
            
            I-AUROC & 0.990 & 0.951 & 0.996 & 0.995 & 0.946 & 0.905 & 0.989 & 0.924 & 0.986 & 0.900 & 0.958 \\
            P-AUROC & 0.996 & 0.995 & 0.999 & 0.974 & 0.982 & 0.980 & 0.999 & 0.998 & 0.998 & 0.996 & 0.992 \\
            AUPRO@30\% & 0.977 & 0.972 & 0.982 & 0.945 & 0.937 & 0.917 & 0.982 & 0.981 & 0.976 & 0.976 & 0.964 \\
            AUPRO@1\%  & 0.455 & 0.423 & 0.482 & 0.458 & 0.367 & 0.330 & 0.480 & 0.469 & 0.465 & 0.445 & 0.437 \\
            
            \hline

            & \multicolumn{10}{c}{\textbf{(d) MLP Projection [CLIP \& Point-MAE] @50ep}} & \\

            \hline

            I-AUROC & 0.893 & 0.778 & 0.865 & 0.989 & 0.940 & 0.777 & 0.726 & 0.828 & 0.948 & 0.591 & 0.833 \\
            P-AUROC & 0.994 & 0.977 & 0.996 & 0.968 & 0.977 & 0.964 & 0.990 & 0.997 & 0.997 & 0.978 & 0.984 \\
            AUPRO@30\% & 0.964 & 0.921 & 0.979 & 0.935 & 0.917 & 0.864 & 0.961 & 0.979 & 0.966 & 0.929 & 0.942 \\
            AUPRO@1\%  & 0.347 & 0.288 & 0.450 & 0.421 & 0.304 & 0.222 & 0.322 & 0.445 & 0.423 & 0.234 & 0.346 \\

            \hline
                        
        \end{tabular}}
    \caption{Best results in \textbf{bold}, runner-ups \underline{underlined}.}
    \label{tab:ftn_backbone_ablation}
\end{table}

==> tables/ftn_cross_modality_ablation_old.tex <==
\begin{table}[h]
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{c||cccccccccc||c}

            \textbf{Metric} &
            \textit{Bagel} &
            \textit{Cable Gland} &
            \textit{Carrot} &
            \textit{Cookie} &
            \textit{Dowel} &
            \textit{Foam} &
            \textit{Peach} &
            \textit{Potato} &
            \textit{Rope} &
            \textit{Tire} &
            \textbf{Mean} \\ 

            \hline

            & \multicolumn{10}{c}{\textbf{(a) MLP Projection [Same Modality, 2D Only] @50ep}} & \\

            \hline
            
            I-AUROC & 0.964 & 0.874 & 0.939 & 0.809 & 0.984 & 0.799 & 0.908 & 0.606 & 0.971 & 0.750 & 0.860 \\
            P-AUROC & 0.992 & 0.988 & 0.994 & 0.942 & 0.968 & 0.942 & 0.995 & 0.993 & 0.996 & 0.987 & 0.980 \\
            AUPRO@30\% & 0.959 & 0.955 & 0.974 & 0.869 & 0.895 & 0.813 & 0.978 & 0.965 & 0.966 & 0.950 & 0.932 \\
            AUPRO@1\%  & 0.393 & 0.400 & 0.417 & 0.263 & 0.277 & 0.283 & 0.453 & 0.358 & 0.425 & 0.340 & 0.361 \\
            
            \hline

            & \multicolumn{10}{c}{\textbf{(b) MLP Projection [Same Modality, 3D Only] @50ep}} & \\

            \hline
            
            I-AUROC & 0.921 & 0.568 & 0.969 & 0.957 & 0.783 & 0.758 & 0.703 & 0.958 & 0.984 & 0.557 & 0.816 \\
            P-AUROC & 0.990 & 0.927 & 0.998 & 0.958 & 0.963 & 0.913 & 0.993 & 0.998 & 0.997 & 0.964 & 0.970 \\
            AUPRO@30\% & 0.969 & 0.746 & 0.981 & 0.929 & 0.884 & 0.679 & 0.974 & 0.981 & 0.970 & 0.890 & 0.900 \\
            AUPRO@1\% & 0.419 & 0.081 & 0.473 & 0.451 & 0.260 & 0.265 & 0.404 & 0.477 & 0.466 & 0.180 & 0.348 \\
            
            \hline

            & \multicolumn{10}{c}{\textbf{(c) MLP Projection [Same Modality, 2D + 3D] @50ep}} & \\

            \hline
            
            I-AUROC & 0.980 & 0.789 & 0.967 & 0.965 & 0.919 & 0.815 & 0.902 & 0.938 & 0.987 & 0.719 & 0.898 \\
            P-AUROC & 0.997 & 0.971 & 0.998 & 0.974 & 0.977 & 0.992 & 0.997 & 0.999 & 0.999 & 0.990 & 0.989 \\
            AUPRO@30\% & 0.980 & 0.918 & 0.982 & 0.950 & 0.923 & 0.966 & 0.981 & 0.982 & 0.980 & 0.966 & 0.963 \\
            AUPRO@1\%  & 0.472 & 0.304 & 0.483 & 0.446 & 0.339 & 0.396 & 0.474 & 0.490 & 0.477 & 0.380 & 0.426 \\
            
            \hline

            & \multicolumn{10}{c}{\textbf{(d) MLP Projection [Cross Modality, 2D + 3D] @50ep}} & \\

            \hline
            
            I-AUROC & 0.990 & 0.894 & 0.986 & 0.989 & 0.980 & 0.916 & 0.951 & 0.916 & 0.986 & 0.886 & 0.949 \\
            P-AUROC & 0.997 & 0.989 & 0.999 & 0.971 & 0.985 & 0.992 & 0.998 & 0.999 & 0.998 & 0.996 & 0.992 \\
            AUPRO@30\% & 0.979 & 0.963 & 0.982 & 0.940 & 0.944 & 0.961 & 0.980 & 0.983 & 0.972 & 0.980 & 0.968 \\
            AUPRO@1\%  & 0.469 & 0.402 & 0.486 & 0.450 & 0.380 & 0.397 & 0.463 & 0.490 & 0.453 & 0.463 & 0.445 \\
            
            \hline
            
        \end{tabular}}
    \caption{Best results in \textbf{bold}, runner-ups \underline{underlined}.}
    \label{tab:ftn_crossmodality_ablation}
\end{table}

==> tables/ftn_few-shot_ablation_old.tex <==
\begin{table}[h]
    \centering
    \resizebox{0.75\linewidth}{!}{%
        \begin{tabular}{c||cccc}

            \textbf{Method} &
            \textit{5-shot} &
            \textit{10-shot} &
            \textit{50-shot} &
            \textit{Full} \\
            
            \hline
            
            & \multicolumn{3}{c}{\textbf{(a) I-AUROC}} & \\

            \hline
            
            BTF~\cite{horwitz2023back}     & 0.671 & \underline{0.695} & 0.806 & 0.865 \\
            AST~\cite{RudWeh2023}          & 0.680 & 0.689 & 0.794 & 0.937 \\
            M3DM~\cite{wang2023multimodal} & \textbf{0.822} & \textbf{0.845} & \textbf{0.907} & \underline{0.945} \\
            Ours                           & \underline{0.811} & \textbf{0.845} & \underline{0.906} & \textbf{0.954} \\
            
            \hline

            & \multicolumn{3}{c}{\textbf{(d) P-AUROC}} & \\

            \hline

            BTF~\cite{horwitz2023back}     & 0.980 & 0.983 & \underline{0.989} & \underline{0.992} \\
            AST~\cite{RudWeh2023}          & 0.950 & 0.946 & 0.974 & 0.976 \\
            M3DM~\cite{wang2023multimodal} & \underline{0.984} & \underline{0.986} & \underline{0.989} & \underline{0.992} \\
            Ours                           & \textbf{0.986} & \textbf{0.987} & \textbf{0.991} & \textbf{0.993} \\

            \hline
            
            & \multicolumn{3}{c}{\textbf{(b) AUPRO@30\%}} & \\

            \hline

            BTF~\cite{horwitz2023back}     & 0.920 & 0.928 & 0.947 & 0.959 \\
            AST~\cite{RudWeh2023}          & 0.903 & 0.835 & 0.929 & 0.944 \\
            M3DM~\cite{wang2023multimodal} & \underline{0.937} & \underline{0.943} & \underline{0.955} & \underline{0.964} \\
            Ours                           & \textbf{0.949} & \textbf{0.954} & \textbf{0.965} & \textbf{0.971} \\
            
            \hline
            
            & \multicolumn{3}{c}{\textbf{(c) AUPRO@1\%}} & \\

            \hline

            BTF~\cite{horwitz2023back}     & 0.288 & 0.308 & 0.356 & 0.383 \\
            AST~\cite{RudWeh2023}          & 0.158 & 0.174 & 0.335 & \underline{0.398} \\
            M3DM~\cite{wang2023multimodal} & \underline{0.330} & \underline{0.355} & \underline{0.387} & 0.394 \\
            Ours                           & \textbf{0.382} & \textbf{0.398} & \textbf{0.431} & \textbf{0.455} \\
            
            \hline
            
        \end{tabular}}
    \caption{\textbf{Few-shot setting performance on MVTec 3D-AD dataset with several AD methods.} Best results in \textbf{bold}, runner-ups \underline{underlined}.}
    \label{tab:ftn_few-shot_mvtec}
\end{table}

==> tables/iauroc_comparisons_eyecandies.tex <==
\begin{table*}
    \centering
    \resizebox{0.75\textwidth}{!}{%
        \begin{tabular}{c||cccccccccc||c}

            \textbf{Method} &
            \textit{Can. C.} &
            \textit{Cho. C.} &
            \textit{Cho. P.} &
            \textit{Conf.} &
            \textit{Gum. B.} &
            \textit{Haz. T.} &
            \textit{Lic. S.} &
            \textit{Lollip.} &
            \textit{Marsh.} &
            \textit{Pep. C.} &
            \textbf{Mean} \\

            \hline

            RGB-D~\cite{bonfiglioli2022eyecandies}    & 0.529 & 0.861 & 0.739 & 0.752 & 0.594 & 0.498 & 0.679 & 0.651 & 0.838 & 0.750 & 0.689 \\
            RGB-cD-n~\cite{bonfiglioli2022eyecandies} & 0.596 & 0.843 & 0.819 & 0.846 & 0.833 & 0.550 & 0.750 & 0.846 & 0.940 & 0.848 & 0.787 \\
            M3DM~\cite{wang2023multimodal}            & 0.624 & 0.958 & 0.958 & 1.000 & 0.886 & 0.758 & 0.949 & 0.836 & 1.000 & 1.000 & 0.897 \\
            % EasyNet~\cite{chen2023easynet}            & 0.737 & 0.934 & 0.866 & 0.966 & 0.717 & 0.822 & 0.847 & 0.863 & 0.977 & 0.960 & 0.869 \\
            Ours                                      & 0.680 & 0.931 & 0.952 & 0.880 & 0.865 & 0.782 & 0.917 & 0.840 & 0.998 & 0.962 & 0.881 \\
            
            \hline
            
        \end{tabular}}
    \caption{I-AUROC on Eyecandies dataset with several models. Best results in \textbf{bold}, runner-ups \underline{underlined}.}
    \label{tab:iauroc_comparisons_eyecandies}
\end{table*}

==> tables/iauroc_comparisons_mvtec.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{0.75\textwidth}{!}{%
        \begin{tabular}{c||cccccccccc||c}

            \textbf{Method} &
            \textit{Bagel} &
            \textit{Cable Gland} &
            \textit{Carrot} &
            \textit{Cookie} &
            \textit{Dowel} &
            \textit{Foam} &
            \textit{Peach} &
            \textit{Potato} &
            \textit{Rope} &
            \textit{Tire} &
            \textbf{Mean} \\ 

            \hline
            DepthGAN~\cite{bergmann2022mvtec} & 0.538 & 0.372 & 0.580 & 0.603 & 0.430 & 0.534 & 0.642 & 0.601 & 0.443 & 0.577 & 0.532 \\
            DepthAE~\cite{bergmann2022mvtec}  & 0.648 & 0.502 & 0.650 & 0.488 & 0.805 & 0.522 & 0.712 & 0.529 & 0.540 & 0.552 & 0.595 \\
            DepthVM~\cite{bergmann2022mvtec}  & 0.513 & 0.551 & 0.477 & 0.581 & 0.617 & 0.716 & 0.450 & 0.421 & 0.598 & 0.623 & 0.555 \\
            VoxelGAN~\cite{bergmann2022mvtec} & 0.680 & 0.324 & 0.565 & 0.399 & 0.497 & 0.482 & 0.566 & 0.579 & 0.601 & 0.482 & 0.517 \\
            VoxelAE~\cite{bergmann2022mvtec}  & 0.510 & 0.540 & 0.384 & 0.693 & 0.446 & 0.632 & 0.550 & 0.494 & 0.721 & 0.413 & 0.538 \\
            VoxelVM~\cite{bergmann2022mvtec}  & 0.553 & 0.772 & 0.484 & 0.701 & 0.751 & 0.578 & 0.480 & 0.466 & 0.689 & 0.611 & 0.609 \\
            BTF~\cite{horwitz2023back}        & 0.918 & 0.748 & 0.967 & 0.883 & 0.932 & 0.582 & 0.896 & 0.912 & 0.921 & 0.886 & 0.865 \\
            AST~\cite{RudWeh2023}             & 0.983 & 0.873 & 0.976 & 0.971 & 0.932 & 0.885 & \textbf{0.974} & \textbf{0.981} & \textbf{1.000} & 0.797 & 0.937 \\
            M3DM~\cite{wang2023multimodal}    & \textbf{0.994} & \textbf{0.909} & \underline{0.972} & \underline{0.976} & \underline{0.960} & \textbf{0.942} & \underline{0.973} & 0.899 & 0.972 & \underline{0.850} & \underline{0.945} \\
            % EasyNet~\cite{chen2023easynet}    & 0.991 & 0.998 & 0.918 & 0.968 & 0.945 & 0.945 & 0.905 & 0.807 & 0.994 & 0.793 & 0.926 \\
            Ours                              & \textbf{0.994} & \underline{0.888} & \textbf{0.984} & \textbf{0.993} & \textbf{0.980} & \underline{0.888} & 0.941 & \underline{0.943} & \underline{0.980} & \textbf{0.953} & \textbf{0.954} \\
            
            \hline
            
        \end{tabular}}
    \caption{\textbf{I-AUROC MVTec 3D-AD of multi-modal AD methods.} Best results in \textbf{bold}, runner-ups \underline{underlined}.}
    \label{tab:iauroc_comparisons_mvtec}
\end{table*}

==> tables/memory-banks_occupancy.tex <==
\begin{table*}
    \centering
    \resizebox{0.85\textwidth}{!}{%
        \begin{tabular}{c||cccccccccc||c}

            \textbf{Method} &
            \textit{Bagel} &
            \textit{Cable Gland} &
            \textit{Carrot} &
            \textit{Cookie} &
            \textit{Dowel} &
            \textit{Foam} &
            \textit{Peach} &
            \textit{Potato} &
            \textit{Rope} &
            \textit{Tire} &
            \textbf{Mean} \\ 

            \hline


            BTF (MB)~\cite{horwitz2023back}     & 228.984 & 209.281 & 268.403 & 197.083 & 270.282 & 221.479 & 338.790 & 281.547 & 279.667 & 197.083 & 249.260 \\
            M3DM (GB)~\cite{wang2023multimodal} & 5.580 & 5.122 & 6.569 & 4.824 & 6.615 & 5.421 & 8.292 & 6.891 & 6.845 & 4.824 & 6.098 \\
            
            \hline
            
        \end{tabular}}
    \caption{Size of memory banks on MVTec 3D-AD dataset.}
    \label{tab:memory-banks_occupancy}
\end{table*}

==> tables/pauroc_comparisons_eyecandies.tex <==
\begin{table*}[!h]
    \centering
        \begin{tabular}{c||cccccccccc||c}

            \textbf{Method} &
            \textit{Can. C.} &
            \textit{Cho. C.} &
            \textit{Cho. P.} &
            \textit{Conf.} &
            \textit{Gum. B.} &
            \textit{Haz. T.} &
            \textit{Lic. S.} &
            \textit{Lollip.} &
            \textit{Marsh.} &
            \textit{Pep. C.} &
            \textbf{Mean} \\

            \hline

            RGB-D~\cite{bonfiglioli2022eyecandies}    & 0.973 & 0.927 & 0.958 & 0.945 & 0.929 & 0.806 & 0.827 & 0.977 & 0.931 & 0.928 & 0.920 \\
            RGB-cD-n~\cite{bonfiglioli2022eyecandies} & 0.980 & 0.979 & 0.982 & 0.978 & 0.951 & 0.853 & 0.971 & 0.978 & 0.985 & 0.967 & 0.962 \\
            M3DM~\cite{wang2023multimodal}            & 0.974 & 0.987 & 0.962 & 0.998 & 0.966 & 0.941 & 0.973 & 0.984 & 0.996 & 0.985 & 0.977 \\
            Ours                                      & 0.983 & 0.982 & 0.964 & 0.989 & 0.949 & 0.946 & 0.969 & 0.980 & 0.995 & 0.987 & 0.974 \\
            
            \hline
            
        \end{tabular}
    \caption{P-AUROC on Eyecandies dataset with several models. Best results in \textbf{bold}, runner-ups \underline{underlined}.}
    \label{tab:pauroc_comparisons_eyecandies}
    
\end{table*}
